Changing the Representation: Examining Language Representation for Neural Sign Language Production

Neural Sign Language Production (SLP) aims to automatically translate from spoken language sentences to sign language videos. Historically the SLP task has been broken into two steps; Firstly, translating from a spoken language sentence to a gloss sequence and secondly, producing a sign language video given a sequence of glosses. In this paper we apply Natural Language Processing techniques to the first step of the SLP pipeline. We use language models such as BERT and Word2Vec to create better sentence level embeddings, and apply several tokenization techniques, demonstrating how these improve performance on the low resource translation task of Text to Gloss. We introduce Text to HamNoSys (T2H) translation, and show the advantages of using a phonetic representation for sign language translation rather than a sign level gloss representation. Furthermore, we use HamNoSys to extract the hand shape of a sign and use this as additional supervision during training, further increasing the performance on T2H. Assembling best practise, we achieve a BLEU-4 score of 26.99 on the MineDGS dataset and 25.09 on PHOENIX14T, two new state-of-the-art baselines.

==> sections/Tables/small_table.tex <==
%phix
\begin{table*}
\centering
\label{pheonix_baseline}
\begin{tabular}{r|ccc} 
\toprule
\multicolumn{1}{l}{}           & \multicolumn{3}{c}{DEV SET}                       \\
\multicolumn{1}{c|}{Approach:} & BLEU-4         & BLEU-1         & ROUGE           \\ 
\hline
T2G \cite{stoll2018sign}                            & 16.34          & 50.15          & 48.42           \\
T2G \cite{saunders2020progressive}                         & 20.23          & 55.65          & 55.41           \\
T2G \cite{li2021transcribing}                           & 18.89          & -              & 49.91           \\
T2G \cite{moryossef2021data}                           & 23.17          & -              & -               \\
                               &                &                &                 \\
\textbf{T2G Baseline (ours)}   & 22.47          & 58.98          & 57.96           \\
\textbf{T2G Best Model (ours)} & \textbf{25.09} & \textbf{60.04} & \textbf{58.82}  \\
\bottomrule
\end{tabular}
\end{table*}


% Mdgs 
\begin{table*}
\centering
\label{tab:text_to_gloss_results}
\begin{tabular}{r|ccc} 
\toprule
\multicolumn{1}{l}{}           & \multicolumn{3}{c}{DEV SET}                       \\
\multicolumn{1}{c|}{Approach:} & BLEU-4         & BLEU-1         & ROUGE           \\ 
\midrule
T2G \cite{saunders2021signing}                           & 3.17           & -              & 32.93           \\
                               &                &                &                 \\
\textbf{T2G Our best}          & 10.5           & 33.56          & 35.79           \\
\textbf{T2G2H Our best}        & 22.06          & 47.55          & 36.20           \\
\textbf{T2H Our best}          & \textbf{26.99} & \textbf{42.73} & \textbf{48.89}  \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}
\centering
\label{tab:translation_with_supervision}
\begin{tabular}{r|c|ccc} 
\toprule
\multicolumn{1}{l}{}           & \multicolumn{1}{l}{} & \multicolumn{3}{c}{DEV SET}                                         \\
\multicolumn{1}{c|}{Approach:} & Supervision          & BLEU-4               & BLEU-1               & ROUGE                 \\ 
\midrule
T2G2H                          & \xmark                     & \textbf{22.06}       & \textbf{47.55}       & \textbf{35.74}        \\
T2G2H                          & \cmark                     & 21.79                & 46.21                & 35.99                 \\ 
\hline
\multicolumn{1}{l}{}           & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  \\
T2H                            & \xmark                     & 26.14                & \textbf{44.35}       & \textbf{50.05}        \\
T2H                            & \cmark                     & \textbf{26.99}       & 42.73                & 48.85                 \\
\bottomrule
\end{tabular}
\end{table*}
